Inverse Resistive Force Theory (I-RFT): Learning granular properties through robot-terrain physical interactions

For robots to navigate safely and efficiently on soft, granular terrains, it is crucial to gather information about the terrain's mechanical properties, which directly affect locomotion performance. Recent research has developed robotic legs that can accurately sense ground reaction forces during locomotion. However, existing tests of granular property estimation often rely on specific foot trajectories, such as vertical penetration or horizontal shear, limiting their applicability during natural locomotion. To address this limitation, we introduce a physics-informed machine learning framework, Inverse Resistive Force Theory (I-RFT), which integrates the Granular Resistive Force Theory model with Gaussian Processes to infer terrain properties from proprioceptively measured contact forces under arbitrary gait trajectories. By embedding the granular force model within the learning process, I-RFT preserves physical consistency while enabling generalization across diverse motion primitives. Experimental results demonstrate that I-RFT accurately estimates terrain properties across multiple gait trajectories and toe shapes. Moreover, we show that the quantified uncertainty over the terrain resistance stress map could enable robots to optimize foot design and gait trajectories for efficient information gathering. This approach establishes a new foundation for data-efficient characterization of complex granular environments and opens new avenues for locomotion strategies that actively adapt gait for autonomous terrain exploration.

==> paper-template-latex/additionalandextensionstudy.tex <==
\section{Additional studies and discussion} 
\subsection{Structural prior incorporation}
As established in~\cite{lichenrft}, the stress per unit depth map $\alpha_{z,x}(\beta, \gamma)$ is generic across dry homogeneous granular media, differing only by a scaling factor $\zeta$. To leverage this prior information, we model terrain-specific stresses as a scaled generic profile plus a GP residual with the initial assumption of dry homogeneous media. Specificalzly, we decompose each stress per unit depth map as:
\begin{align}
\alpha_z(\theta) &= \zeta_z \cdot \alpha_{\text{base},z}(\theta) + r_z(\theta), \nonumber \\
&\quad r_z(\cdot) \sim \mathcal{GP}(0, k_z(\cdot, \cdot)), \\
\alpha_x(\theta) &= \zeta_x \cdot \alpha_{\text{base},x}(\theta) + r_x(\theta), \nonumber \\
&\quad r_x(\cdot) \sim \mathcal{GP}(0, k_x(\cdot, \cdot)),
\end{align}
where $\alpha_{\text{base},z}(\theta)$ and $\alpha_{\text{base},x}(\theta)$ are the known generic profiles reported in~\cite{lichenrft}, $\zeta_z$ and $\zeta_x$ are terrain-specific scaling factors, and $r_z(\theta)$ and $r_x(\theta)$ are residual GP functions using the same kernel structure as defined in Sec. \ref{sec-gaussian}.

Substituting this decomposition into the composite observation model (Eq.~\eqref{eq:rft_sensor_integration}), each torque observation becomes a combination of the scaled base profile contribution and the residual GP evaluations. We define residual observations as $\mathbf{y}(\zeta) \triangleq \boldsymbol{\tau}_t - \boldsymbol{\tau}_{\text{base}}(\zeta)$, where $\boldsymbol{\tau}_{\text{base}}(\zeta)$ is the torque predicted by the scaled generic profile alone. The residual model then follows the same composite observation structure as before: $\mathbf{y} \sim \mathcal{N}(\mathbf{0}, C)$ where $C = W_z K_z W_z^\top + W_x K_x W_x^\top + \sigma_n^2 I$ (same as Eq.~\eqref{eq:joint_distribution_composite}).

In practice, we fit this semi-parametric model hierarchically. In the \emph{first stage}, we set $r_z = r_x = 0$ and estimate the scaling factors by minimizing the discrepancy between the measured torques and the torques predicted by the scaled base profile,
\begin{equation}
(\hat{\zeta}_z, \hat{\zeta}_x)
= \arg\min_{\zeta_z, \zeta_x}
\big\|\boldsymbol{\tau}_t - \boldsymbol{\tau}_{\text{base}}(\zeta)\big\|_2^2,
\end{equation}
which is equivalent to maximum likelihood under a Gaussian noise model with no residual GP. In the \emph{second stage}, we fix $\zeta = \hat{\zeta}$ and treat $\mathbf{y}(\hat{\zeta})$ as observations of the residual GP, using the composite covariance $C$ defined above. The residual GP hyperparameters $\psi = \{\ell_z, \ell_x, \sigma_{f,z}, \sigma_{f,x}, \sigma_{n, z}, \sigma_{n, x}\}$ are then optimized following Eqn. \ref{eq:marginal_log_likelihood}. 

This hierarchical formulation is designed to be numerically stable and interpretable: the scaling factors $\hat{\zeta}_z$ and $\hat{\zeta}_x$ capture global material strength with the assumption of dry homogeneous media, while the residual GP is used only to discover new effects in an unknown granular terrain from the RFT prior, such as anisotropy, cohesion, saturation effects, or other non-RFT behaviors.



% \subsection{Active Learning to Improve Performance}
% Based on the derivations above, obtaining a more accurate stress map requires that, during data collection, we acquire angle parameters $\theta$ that are distributed as broadly as possible. This guides how we choose the leg shape and motion mode so as to maximize data efficiency.




\subsection{Incorporating strong priors and hypothesis verification}
\subsection{4. Incorporating Structured Priors into a Semi-Parametric Residual GP}

To enhance model robustness and interpretability, we incorporate structured prior information derived from prior terrain knowledge or a reference model. We define:

\[
f(\theta) = a \cdot f_{\text{base}}(\theta) + r(\theta), \quad r(\cdot) \sim \mathcal{GP}(0, k(\cdot, \cdot)),
\]

where the residual function $r(\theta)$ captures deviations from the base function. The composite observations then become:

\[
y_i = \sum_{m=1}^{M} w_{i,m}[a \cdot f_{\text{base}}(\theta_{i,m}) + r(\theta_{i,m})] + \varepsilon_i.
\]

Letting $\mathbf{f}_{\text{base}}$ represent the vector of base function evaluations and $\mathbf{r}$ the residual latent function, we express the marginal log-likelihood as:

\begin{align}
\log p(\mathbf{y}_t \mid a)
&= -\frac{1}{2} 
    (\mathbf{y}_t - a W\mathbf{f}_{\text{base}})^\top \nonumber \\
&\quad \cdot (W K W^\top + \sigma_n^2 I)^{-1}
    (\mathbf{y}_t - a W\mathbf{f}_{\text{base}}) \nonumber \\
&\quad - \frac{1}{2} 
    \log \!\left| W K W^\top + \sigma_n^2 I \right| 
    - \frac{t}{2} \log(2\pi).
\end{align}



Optimizing this likelihood jointly over the scaling factor $a$ and GP hyperparameters yields a flexible and adaptive model. This approach explicitly quantifies structured deviations from prior knowledge, providing valuable insights into the validity and applicability of the prior.

\subsection{Active trajectory design and shape selection}
{\SL more ablation study comes here}

\section{Real Robot experiments}
{\SL needs an image for the Real Robot setup and comparisons}
\subsection{Experiments of customized motion primitives}
\subsubsection{Traveler robotic leg}
\subsubsection{Experiment setup}
\subsubsection{Estimation results}
\subsubsection{Analysis}
\subsection{Experiments of C-shape leg and rotating motion primitives}

\subsection{Proprioceptive Sensory Modeling}

During locomotion, we observe proprioceptive measurements as motor torques \(\boldsymbol{\tau} = [\tau_1, \tau_2, \dots, \tau_N]^\top\), a vector of observed torque estimations where each element corresponds to a motor, estimated from motor current using the torque constant~\cite{kenneally2016design}. External contact forces \(\mathbf{F}_{\text{external}} = [f_x, f_z]^\top\) acting on the robot are transformed through the robot's kinematic Jacobian \(\mathbf{J}\) to produce these joint-level torques:
\begin{equation}
\boldsymbol{\tau} = \mathbf{J}^{\top} \mathbf{F}_{\text{external}}
\label{eq:jacobian_transform}
\end{equation}
where \(\mathbf{F}_{\text{external}}\) represents contact forces in the robot frame. The Jacobian derivation for the four robot configurations used in this paper is provided in Appendix~\ref{app:jacobian}.

To integrate this sensory model with RFT, the joint torques \(\boldsymbol{\tau}\) arise from the integral of local stress contributions across all contact segments, each transformed through its segment-specific Jacobian:
\begin{equation}
\boldsymbol{\tau} = \sum_{m=1}^{M} |z_m| A_m \, \mathbf{J}_m^{\top} \begin{bmatrix} \alpha_z(\beta_m, \gamma_m) \\ \alpha_x(\beta_m, \gamma_m) \end{bmatrix}
\label{eq:rft_sensor_integration}
\end{equation}
where \(\mathbf{J}_m \in \mathbb{R}^{2 \times N}\) is the Jacobian for the \(m\)-th segment (mapping 2D contact forces to \(N\) joint torques), and \(\boldsymbol{\tau} \in \mathbb{R}^{N}\) is the vector of joint torques. During interaction, \(|z_m|\), \(A_m\), and \(\mathbf{J}_m\) are known from the robot's state and contact geometry, while they vary with segment and robot configuration. 

The Jacobian transformation couples the vertical and horizontal stress components: each torque observation \(\tau_i\) is a linear combination of both \(\alpha_z\) and \(\alpha_x\) evaluated at multiple segments. While we model \(\alpha_z\) and \(\alpha_x\) as independent Gaussian processes, the joint torque observations require solving them jointly, as the Jacobian matrix \(\mathbf{J}_m\) simultaneously transforms both force components into the observed torques. This formulation couples the RFT forward model with the proprioceptive sensor model, forming a linear inverse problem to infer the latent stress per unit depth maps \(\alpha_z(\beta, \gamma)\) and \(\alpha_x(\beta, \gamma)\) from joint-level torque observations \(\boldsymbol{\tau}\).


\newpage
\appendix

\section{Jacobian Derivation}
\label{app:jacobian}

This appendix provides the Jacobian derivation for the four robot configurations used in this paper. The Jacobian matrix relates joint-level torques to end-effector forces, enabling the transformation from proprioceptive measurements to contact forces.

\subsection{Traveler Leg Configuration}

For the Traveler leg configuration, the Jacobian derivation follows the kinematic relationships shown in Fig.~\ref{fig:traveler}. The end-effector position \((x, y)\) is expressed in terms of the composite length \(l\) and angle \(\theta\):
\[
x = l \sin(\theta), \quad y = l \cos(\theta),
\]
where \(l = l_3 + l_1 \cos(\gamma) + \sqrt{l_2^2 - l_1^2 \sin^2(\gamma)}\), and the angles are defined as:
\[
\theta = \frac{1}{2}(\phi_1 + \phi_2), \quad \gamma = \frac{1}{2}(-\phi_1 + \phi_2),
\]
with \(\phi_1\) and \(\phi_2\) being the joint angles.

The differential kinematics relating end-effector position to joint angles is:
\[
\begin{bmatrix} dx \\ dy \end{bmatrix} = \mathbf{J} \begin{bmatrix} d\phi_1 \\ d\phi_2 \end{bmatrix},
\]
where the Jacobian matrix \(\mathbf{J}\) is:
\[
\mathbf{J} = \frac{1}{2} \begin{bmatrix}
-\Phi \sin(\theta) + l \cos(\theta) & \Phi \sin(\theta) + l \cos(\theta) \\
-\Phi \cos(\theta) - l \sin(\theta) & \Phi \cos(\theta) - l \sin(\theta)
\end{bmatrix},
\]
with \(\Phi = -l_1 \sin(\gamma) \left(1 + \frac{l_1 \cos(\gamma)}{\sqrt{l_2^2 - l_1^2 \sin^2(\gamma)}}\right)\).

Using the principle of virtual work, the relationship between end-effector forces and joint torques is:
\[
\begin{bmatrix} F_x \\ F_y \end{bmatrix} = \begin{bmatrix} \tau_1 \\ \tau_2 \end{bmatrix} \mathbf{J}^{-1},
\]
where \(F_x\) and \(F_y\) are the leg forces exerted on the substrate, and \(\tau_1\) and \(\tau_2\) are the joint torques. This result does not include gravity compensation.

\subsection{Other Configurations}

The Jacobian derivations for the remaining three robot configurations (C-leg rotation, plate toe with Traveler leg, and C-toe with Traveler leg) follow similar principles, with the specific kinematic relationships depending on each configuration's geometry and degrees of freedom.


\subsection{Proprioceptive Sensory Modeling}

During locomotion, we observe proprioceptive measurements as motor torques \(\boldsymbol{\tau} = [\tau_1, \tau_2, \dots, \tau_N]^\top\), a vector of observed torque estimations where each element corresponds to a motor, estimated from motor current using the torque constant~\cite{kenneally2016design}. External contact forces \(\mathbf{F}_{\text{external}} = [f_x, f_z]^\top\) acting on the robot are transformed through the robot's kinematic Jacobian \(\mathbf{J}\) to produce these joint-level torques:
\begin{equation}
\boldsymbol{\tau} = \mathbf{J}^{\top} \mathbf{F}_{\text{external}}
\label{eq:jacobian_transform}
\end{equation}
where \(\mathbf{F}_{\text{external}}\) represents contact forces in the robot frame. The Jacobian derivation for the four robot configurations used in this paper is provided in Appendix~\ref{app:jacobian}.

To integrate this sensory model with RFT, the joint torques \(\boldsymbol{\tau}\) arise from the integral of local stress contributions across all contact segments, each transformed through its segment-specific Jacobian:
\begin{equation}
\boldsymbol{\tau} = \sum_{m=1}^{M} |z_m| A_m \, \mathbf{J}_m^{\top} \begin{bmatrix} \alpha_z(\beta_m, \gamma_m) \\ \alpha_x(\beta_m, \gamma_m) \end{bmatrix}
\label{eq:rft_sensor_integration}
\end{equation}
where \(\mathbf{J}_m \in \mathbb{R}^{2 \times N}\) is the Jacobian for the \(m\)-th segment (mapping 2D contact forces to \(N\) joint torques), and \(\boldsymbol{\tau} \in \mathbb{R}^{N}\) is the vector of joint torques. During interaction, \(|z_m|\), \(A_m\), and \(\mathbf{J}_m\) are known from the robot's state and contact geometry, while they vary with segment and robot configuration. 

The Jacobian transformation couples the vertical and horizontal stress components: each torque observation \(\tau_i\) is a linear combination of both \(\alpha_z\) and \(\alpha_x\) evaluated at multiple segments. While we model \(\alpha_z\) and \(\alpha_x\) as independent Gaussian processes, the joint torque observations require solving them jointly, as the Jacobian matrix \(\mathbf{J}_m\) simultaneously transforms both force components into the observed torques. This formulation couples the RFT forward model with the proprioceptive sensor model, forming a linear inverse problem to infer the latent stress per unit depth maps \(\alpha_z(\beta, \gamma)\) and \(\alpha_x(\beta, \gamma)\) from joint-level torque observations \(\boldsymbol{\tau}\).



1. analysis of different noise levels. 




==> paper-template-latex/inverserft.tex <==
\section{Inverse-RFT}
\label{sec-irft}
\ready{shipeng +1, FQ+1}

\subsection{Problem formulation and Inverse RFT overview}
During robot locomotion, terrain stress maps over local interaction angles $(\beta,\gamma)$ are not directly observable. Instead, we observe only force measurements that aggregate stress contributions from multiple contact segments. To infer terrain mechanical properties from these indirect observations, we formulate the \emph{Inverse RFT} problem: reconstructing terrain stress maps from force observations and robot state.

To address the challenges of (i) modeling forward forces under arbitrary geometries and (ii) handling composite observations, we model latent stress maps as Gaussian processes and leverage RFT to decompose forces into orientation-dependent stress contributions (Section~\ref{sec-probabilistic-modeling}), then derive a posterior predictive distribution for composite observations (Section~\ref{sec-composite}). 

\begin{figure}[h]
  \centering
\includegraphics[width=0.48\textwidth]{imgs/RFT_label_v3.png}
% {\SL We probably don't have to use the image B to explain RFT, WE need a sketch to illustrate how forward RFT works and how I-RFT works}
  \caption{Illustration of RFT method. (A) Example of CToe-terrain interaction. It's discretized into 10 segments and are labeled with index 0 to 9. (B) Zooms in and shows resistive force applied on one segment with geometric parameters. (C) Each segment's interaction angles at the moment. (D) Illustrate the idea of forward process. Each segment contributes to bulk force and is the black mark with index on ground truth stress map.}
  \label{fig:rft}
\end{figure}
\subsection{Probabilistic Modeling}
\label{sec-probabilistic-modeling}

During locomotion, we observe composite external contact forces in the robot frame, denoted as \(\mathbf{F} = [F_z, F_x]^\top\) (vertical then horizontal). These forces arise from the integral of local stress contributions across all contact segments. Specifically, each force vector \(\mathbf{F}_i = [F_{i,z}, F_{i,x}]^\top\) at time step \(i\) follows:
\begin{align}
\mathbf{F}_i &= \sum_{m=1}^{M} |z_{i,m}| A_{i,m} \begin{bmatrix} \alpha_z(\theta_{i,m}) \\ \alpha_x(\theta_{i,m}) \end{bmatrix} + \boldsymbol{\varepsilon}_i, \nonumber \\
\boldsymbol{\varepsilon}_i &\sim \mathcal{N}(\mathbf{0}, \sigma_n^2 I_2),
\label{eq:rft_force_integration}
\end{align}
where \(|z_{i,m}|\) and \(A_{i,m}\) are the known depth and area of the \(m\)-th segment at time step \(i\), \(\theta_{i,m} = (\beta_{i,m}, \gamma_{i,m})\) are the local interaction angles computed from the robot state and contact geometry, and \(\boldsymbol{\varepsilon}_i\) is i.i.d.\ Gaussian noise with variance \(\sigma_n^2\). Each observation \(\mathbf{F}_i\) thus combines evaluations of both \(\alpha_z(\theta)\) and \(\alpha_x(\theta)\) at multiple known angle pairs \(\{\theta_{i,m}\}_{m=1}^{M}\).

Given a dataset comprising multiple composite observations:
\begin{equation}
\mathcal{D}_t = \{(\{\theta_{i,m}\}_{m=1}^{M}, \{w_{i,m}\}_{m=1}^{M}, \mathbf{F}_i)\}_{i=1}^{t},
\label{eq:composite_dataset}
\end{equation}
where \(\mathbf{F}_i \in \mathbb{R}^{2}\) is the composite force vector at time step \(i\). The scalar weights \(w_{i,m} = |z_{i,m}| A_{i,m}\) encode the geometric scaling factors that convert stress per unit depth to force contributions: each weight multiplies the stress map evaluation \(\alpha_z(\theta_{i,m})\) or \(\alpha_x(\theta_{i,m})\) to yield the force contribution from segment \(m\) at time step \(i\), as shown in Eq.~\eqref{eq:rft_force_integration}.

To model the latent stress maps \(\alpha_z(\beta, \gamma)\) and \(\alpha_x(\beta, \gamma)\), we place independent Gaussian process priors over them. To model smooth spatial variation in the stress maps, we use a Radial Basis Function (RBF) kernel. Following the original RFT formulation~\cite{lichenrft}, the stress maps exhibit periodic boundary conditions: $\beta$ has periodicity $\pi$ (i.e., $\beta = 0$ and $\beta = \pi$ represent the same physical configuration), while $\gamma = 0$ and $\gamma = \pi$ represent different cases. To enforce the $\pi$-periodicity in $\beta$, we apply a sinusoidal feature embedding
\[
\phi(\theta) = (\sin(2\beta), \cos(2\beta), \sin(\gamma), \cos(\gamma)),
\]
where the factor of 2 in the $\beta$ terms ensures $\pi$-periodicity, and define the kernel as
\[
k(\theta,\theta') = \sigma_f^2
\exp\!\left(-\frac{1}{2}\sum_{d=1}^{4}
\frac{(\phi_d(\theta)-\phi_d(\theta'))^2}{\ell_d^2}\right),
\]
where $\sigma_f^2$ is the signal variance and $\ell_d$ are dimension-wise lengthscales. 

This formulation represents a \emph{linear inverse problem}~\cite{randrianarisoa2023variational}, where the observations are linear operator evaluations of the latent GP functions. Specifically, each force observation is a linear combination of function evaluations: \(\mathbf{F}_i = \mathcal{L}_i[\alpha_z, \alpha_x] + \boldsymbol{\varepsilon}_i\), where \(\mathcal{L}_i\) is a linear operator that applies the weights \(w_{i,m}\) to evaluate both stress components at multiple angle pairs. The joint probability distribution over these composite observations follows a Gaussian distribution:
\begin{equation}
\mathbf{F}_t \sim \mathcal{N}(\mathbf{0}, W_z K_z W_z^\top + W_x K_x W_x^\top + \sigma_n^2 I),
\label{eq:joint_distribution_composite}
\end{equation}
where the weight matrices $W_z, W_x \in \mathbb{R}^{2t \times tM}$ encode the linear operators mapping the GP function evaluations to observations, and the kernel matrices $K_z, K_x \in \mathbb{R}^{tM \times tM}$ capture the covariance structure of the latent functions:
\begin{align}
(K_z)_{(i,m),(j,m')} &= k_z(\theta_{i,m}, \theta_{j,m'}), \\
(K_x)_{(i,m),(j,m')} &= k_x(\theta_{i,m}, \theta_{j,m'}), \\
(W_z)_{(i,c),(j,m)} &= w_{i,m} \,\delta_{ij} \,\mathbb{I}[c=z], \\
(W_x)_{(i,c),(j,m)} &= w_{i,m} \,\delta_{ij} \,\mathbb{I}[c=x].
\end{align}
Here, indices $i,j \in \{1,\dots,t\}$ denote time steps; 
$m,m' \in \{1,\dots,M\}$ index segments; 
and $c \in \{z,x\}$ indexes the force components.
The Kronecker delta $\delta_{ij}$ equals 1 when 
$i=j$ and 0 otherwise.




% The predictive mean is a weighted combination of the training observations, where the weights depend on the similarity (via the kernel) between \(\theta_*\) and the training inputs. The predictive variance decreases when \(\theta_*\) is close to observed points and increases in regions with sparse observations.


\subsection{Posterior Predictive Distribution with Composite Observation}
\label{sec-composite}
Given the probabilistic model defined in Section~\ref{sec-probabilistic-modeling}, we now derive the posterior predictive distribution of granular terrain properties for making predictions from composite observations. Given a new test input describing a toe-terrain interaction configuration, characterized by a set of angle pairs $\{\theta_*^{(m)} = (\beta_*^{(m)}, \gamma_*^{(m)})\}_{m=1}^{M}$ describing the orientation and movement direction of each contact segment, along with corresponding known geometric weights $\{w_*^{(m)}\}_{m=1}^{M}$ (computed from segment depths $|z_*^{(m)}|$ and areas $A_*^{(m)}$ as in Eq.~\eqref{eq:rft_force_integration}), we can make predictions for the stress map and external forces:

% \textbf{Force prediction:} The predictive distribution for a composite force observation $\mathbf{F}_*$ follows the same structure as the direct observation case described in the previous subsection, with the following modifications for composite observations:
% \begin{itemize}
% \item Instead of a single test point $\theta_*$, we have multiple angle pairs $\{\theta_*^{(m)}\}_{m=1}^{M}$ for $M$ contact segments.
% \item The kernel evaluation $k(\theta_*, \Theta)$ is replaced by the linear operator $(w_{*,z}^\top K_{*,z} + w_{*,x}^\top K_{*,x})$, where $w_{*,z} = [[w_*^{(1)}]_z, \dots, [w_*^{(M)}]_z]^\top$ and $w_{*,x} = [[w_*^{(1)}]_x, \dots, [w_*^{(M)}]_x]^\top$ are weight vectors extracted from the weight matrices, and $(K_{*,z})_{(i,m)} = k_z(\theta_*^{(m)}, \theta_{i,m})$ and $(K_{*,x})_{(i,m)} = k_x(\theta_*^{(m)}, \theta_{i,m})$ are cross-covariance matrices between test and training points.
% \item The covariance matrix $K + \sigma_n^2 I$ is replaced by $W_z K_z W_z^\top + W_x K_x W_x^\top + \sigma_n^2 I$ to account for composite observations.
% \item The prior variance $k(\theta_*, \theta_*)$ is replaced by $w_{*,z}^\top K_{**,z} w_{*,z} + w_{*,x}^\top K_{**,x} w_{*,x}$, where $(K_{**,z})_{mn} = k_z(\theta_*^{(m)}, \theta_*^{(n)})$ and $(K_{**,x})_{mn} = k_x(\theta_*^{(m)}, \theta_*^{(n)})$ are the covariance matrices between test points.
% \end{itemize}

\textbf{Stress map prediction:} The learned stress map $\alpha_z(\theta)$ (and similarly $\alpha_x(\theta)$) is a continuous function over the angle space $\theta = (\beta, \gamma)$. For any test angle pair $\theta_* = (\beta_*, \gamma_*)$, we can predict the stress map value with uncertainty. Since the composite observations aggregate multiple segments, we must account for the full covariance induced by the observation operator when predicting each component. For the vertical component $\alpha_z$, the posterior mean and variance are:
\begin{align}
\mu_{\alpha_z}(\theta_*) &= \mathbf{k}_z(\theta_*, \Theta)^\top W_z^\top \nonumber \\
&\quad \times (W_z K_z W_z^\top + W_x K_x W_x^\top + \sigma_n^2 I)^{-1} \mathbf{F}_t, \label{eq:stress_z_mean} \\
\sigma_{\alpha_z}^2(\theta_*) &= k_z(\theta_*, \theta_*) \nonumber \\
&\quad - \mathbf{k}_z(\theta_*, \Theta)^\top W_z^\top \nonumber \\
&\quad \times (W_z K_z W_z^\top + W_x K_x W_x^\top + \sigma_n^2 I)^{-1} \nonumber \\
&\quad \times W_z \mathbf{k}_z(\theta_*, \Theta), \label{eq:stress_z_var}
\end{align}here $\mathbf{k}_z(\theta_*, \Theta)$ is a column vector of kernel evaluations $[k_z(\theta_*, \theta_{1,1}), \dots, k_z(\theta_*, \theta_{t,M})]^\top$ between the test angle $\theta_*$ and all training angle pairs, $W_z$ and $K_z$ are the weight and kernel matrices for the vertical component, and $\mathbf{F}_t$ contains all composite force observations. The horizontal component $\alpha_x$ follows the same procedure.
% \begin{align}
% \mu_{\alpha_x}(\theta_*) &= \mathbf{k}_x(\theta_*, \Theta)^\top W_x^\top \nonumber \\
% &\quad \times (W_z K_z W_z^\top + W_x K_x W_x^\top + \sigma_n^2 I)^{-1} \mathbf{F}_t, \label{eq:stress_x_mean} \\
% \sigma_{\alpha_x}^2(\theta_*) &= k_x(\theta_*, \theta_*) \nonumber \\
% &\quad - \mathbf{k}_x(\theta_*, \Theta)^\top W_x^\top \nonumber \\
% &\quad \times (W_z K_z W_z^\top + W_x K_x W_x^\top + \sigma_n^2 I)^{-1} \nonumber \\
% &\quad \times W_x \mathbf{k}_x(\theta_*, \Theta), \label{eq:stress_x_var}
% \end{align}
% where the notation is analogous for the horizontal component.

\textbf{Force prediction:} The learned stress map in turn allows prediction of future leg-terrain contact forces $\mathbf{F}_* = [F_{z,*}, F_{x,*}]^\top$ for arbitrary toe-terrain interaction, which is crucial for locomotion adaptation on varying terrain properties. To achieve this, we evaluate the stress map at each segment's angle pair $\theta_*^{(m)} = (\beta_*^{(m)}, \gamma_*^{(m)})$ (where $m = 1, \dots, M$ indexes the segments, each with different orientations along the contact surface), then sum the contributions using the RFT forward model (Eq.~\eqref{eq:rft_discrete}). The predicted mean forces are:
\begin{align}
F_{z,*} &= \sum_{m=1}^{M} |z_*^{(m)}| A_*^{(m)} \mu_{\alpha_z}(\theta_*^{(m)}), \\
F_{x,*} &= \sum_{m=1}^{M} |z_*^{(m)}| A_*^{(m)} \mu_{\alpha_x}(\theta_*^{(m)}),
\end{align}
where $\mu_{\alpha_x}(\theta_*^{(m)})$ is computed analogously to $\mu_{\alpha_z}(\theta_*^{(m)})$ using the horizontal component's matrices and observations. The uncertainty in force predictions propagates from the stress map uncertainties:
\begin{align}
\sigma_{F_z}^2 &= \sum_{m=1}^{M} (|z_*^{(m)}| A_*^{(m)})^2 \sigma_{\alpha_z}^2(\theta_*^{(m)}), \\
\sigma_{F_x}^2 &= \sum_{m=1}^{M} (|z_*^{(m)}| A_*^{(m)})^2 \sigma_{\alpha_x}^2(\theta_*^{(m)}),
\end{align}
where we assume independence between segments for uncertainty propagation. With composite observations, the marginal log-likelihood of the force observations $\mathbf{F}_t \in \mathbb{R}^{2t}$ becomes:
\begin{align}
\log p(\mathbf{F}_t)
&= \underbrace{-\frac{1}{2}\,\mathbf{F}_t^\top (W_z K_z W_z^\top + W_x K_x W_x^\top + \sigma_n^2 I)^{-1} \mathbf{F}_t}_{\text{model fit}} \nonumber \\
&\quad \underbrace{- \frac{1}{2} \log \left| W_z K_z W_z^\top + W_x K_x W_x^\top + \sigma_n^2 I \right|}_{\text{model complexity}} \nonumber \\
&\quad \underbrace{- \frac{tN}{2} \log(2\pi)}_{\text{constant}}. \label{eq:marginal_log_likelihood}
\end{align}



==> paper-template-latex/relatework.tex <==
\section{Related Work}
% {\SL Feng, you can follow the order of five item to draft a survey, add citations.}
% \begin{itemize}
%     \item Terradynamics - a survey, why we want to use RFT as our basis to estimate terrain. 
%     \item Robot Terrain Sensing - a survey ( most of the robot use vision or proprioceptive information to classify terrain, or use simple protocols e.g., penetration to characterize the terrain; we lack a way to infer terrain in arbitrary gaits)
%     \item Gaussian Processes for Composite Observations (doing a survey of Multi-output GPs, Linear-transformation GPs, Convolved GPs; Standard GP regression assumes pointwise observations of the function. In contrast, our measurements are summed contributions from multiple contact patches with different angles, requiring a composite-kernel GP, so we create a composite-kernel combining robot kinematics and state information. 
%     \item active learning \& adaptive informative planning: doing a survey about Active perception in robotics, Info-gain optimization (entropy, mutual information, expected improvement) to talk about active trajectory/gait design -> informative-guided locomotion. 
% \end{itemize}
\subsection{Granular Terradynamics and Resistance Force Theory (RFT)}
% {\SL too much words on DEM , MGM, SPH METHODS, this can be reduced into one group, and clearly stating their drawback, for RFT, there are a few works including 3d-rft, dynamic RFT, and finally, a few sentences why we chose rft as our latent for robotic applications.}
Due to its distinctive solid–fluid characteristics, the granular terrain often interacts with robots in complex and difficult-to-predict ways. 
% Early work was mainly empirical and based on classical mechanics, developed for heavy wheeled or tracked vehicles.\cite{WONG1984117} These approaches are limited to simple contact conditions and cannot be generalized to complex legged locomotion patterns. 
High-fidelity numerical methods have been widely explored. Discrete Element Method (DEM) simulations explicitly resolve grain–grain and grain–intruder contacts and can reproduce detailed force histories and substrate deformation for legged and wheeled locomotion\cite{SMITH2013277, Qian_walking}.
% More recently, continuum approaches that treat dense granular media as frictional, non-Newtonian continua have better efficiency. Agarwal et al. prove this method implemented with Material Point Method (MGM) can capture a broad range of intrusion problems, including wheel locomotion\cite{AGARWAL20191} and dynamic impacts near free surfaces.\cite{simplicity}
Wang et al. first introduce Smooth Particle Hydrodynamics (SPH) method\cite{WANG20172439} to terradynamics and prove its high fidelity.
While DEM and continuum models are powerful and increasingly general, they remain computationally expensive, require substantial parameter identification, and are not well suited for model-based control, or real-time planning and measurement.

An alternative line of work adapts resistive force theory (RFT). Li et al. established this "granular RFT"\cite{lichenrft} and demonstrated that experimentally measured local stress profiles can be integrated to predict the forces on arbitrarily shaped legs, thereby enabling the first quantitative "terradynamics" of legged locomotion on granular media. 
Later scholars extend the resistive force theory to 3D space\cite{3d-rft}, proving that the theory can adapt to more complex gaits or motion modes. 
Agarwal et al\cite{simplicity} further this theory, which was originally formulated under a quasi-static motion assumption, to cases that are applicable to high-speed motion. This dynamic RFT research enable better states estimation for real world legged robots. 
In this work, we adopt granular RFT as our theoretical foundation for lower computational cost with a clear mechanical interpretation.

% While RFT models provide useful approximations in many natural substrates, estimating the stress per unit depth map \(\alpha_{z,x}(\beta, \gamma)\) empirically for different terrains remains a challenge. Traditional experimental measurements, due to mechanical constraints, can only obtain discrete maps like Fig.\ref{fig:rft}A,B, and for certain \((\beta, \gamma)\) values are difficult to measure.



\subsection{Terrain Sensing and Characterization}
% {\SL the cite symbol ~\cite{} needs to be on the front of dot. and the force estimation is not our final goal, so the logic is a little bit unclear here. 2. when you say the proprioceptive methods cannot accurately estimate the net force on legs, do you propose a way to solve this problem in this paper, I think this is not the problem we are going to solve, so this reasoning logic need to be changed. }
Current mainstream terrain sensing can be broadly divided into non-contact sensing and proprioceptive sensing. 
Non-contact sensing mostly based on camera\cite{MarsVisionClassification,visionTerrainEstimation,semanticsensing}. These methods adopt semantic segmentation and vision-based terrain classification, and then use existing data to estimate the mechanical properties of the ground. However, these approaches are highly susceptible to environmental interference and cannot account for variations caused by factors such as compaction, moisture content. They also can't provide reliable quantitative force estimation.
Proprioceptive methods use intrinsic proprioceptive sensors (motor current, IMU, tactile, and Force/Torque sensors)\cite{bevameter,hutterhaptics,valada} and usually have higher accuracy. These methods can more accurately estimate the robot’s state or classify the terrain, but they still cannot directly measure the mechanical properties of the terrains. Consequently, we are unable to infer more complex robot–ground interaction forces using these approaches, nor to use such force estimates as a basis for planning and control.
\\
\subsection{Linear inverse problems and probabilistic modeling}
\begin{itemize}
    \item basic GP and capabilities
    \item limitations, related to our problem
    \item recent progress in linear inverse algorithms
\end{itemize}
{\SL similarly, cite need to be place before dot symbol., introduce linear inverse problem papers, let's introduce different ways of solve it and also do a literature review on different model ways, and there advantages and disadvantages. Finally, provide a logic why we chose Gaussian process. }
Following the idea proposed by Krotkov et al.\cite{Krotkov-1990-13157}, we aim for the robot to efficiently gather information during its exploration process,  which is a foundational research topic that answers how a robot (team) can efficiently build an accurate model of an unknown target function\cite{Chen_2023} \cite{JMLR:v12:alvarez11a}.
some paper resources I can find (commented):
% https://proceedings.neurips.cc/paper_files/paper/2023/file/5c25c15b5b2fd386ab188a918e54c7d5-Paper-Conference.pdf
% https://arxiv.org/pdf/2311.00663
% https://arxiv.org/pdf/2502.04276
% https://proceedings.neurips.cc/paper_files/paper/2023/file/9c70cfa2e7d9328c649c94d50cbf8faf-Paper-Conference.pdf
% (some diffusion works, etc)
\\


% We propose a method based on inverse RFT. By collecting the contact forces under a specific gait, we obtain a stress map of the terrain, which allows us to estimate the forces for arbitrary foot shapes and gaits. To learn this complex mapping, we employ Gaussian process regression. Standard GP regression assumes point-wise observations of the function.\cite{GPMIT} In contrast, our measurements are summed contributions from multiple contact patches with different angles, requiring a composite-kernel GP, so we create a composite-kernel combining robot kinematics and state information.


